In the IP of the Beholder: Strategies for Active IPv6 Topology Discovery

Existing methods for active topology discovery within the IPv6 Internet largely mirror those of IPv4. In light of the large and sparsely populated address space, in conjunction with aggressive ICMPv6 rate limiting by routers, this work develops a different approach to Internet-wide IPv6 topology mapping. We adopt randomized probing techniques in order to distribute probing load, minimize the effects of rate limiting, and probe at higher rates. Second, we extensively analyze the efficiency and efficacy of various IPv6 hitlists and target generation methods when used for topology discovery, and synthesize new target lists based on our empirical results to provide both breadth (coverage across networks) and depth (to find potential subnetting). Employing our probing strategy, we discover more than 1.3M IPv6 router interface addresses from a single vantage point. Finally, we share our prober implementation, synthesized target lists, and discovered IPv6 topology results.

==> results_too_table_scaled.tex <==

% DO NOT EDIT MANUALLY!
% CREATED AUTOMATICALLY FROM "results_too_table.tex"

\begin{table*}[t]
  \caption{Additional results, reverse sorted by number of (unique) Hop Router Addrs, \ie yield of routers discovered.}\label{tab:results_too}
  \vspace{-4mm}
  \begin{center}
  \begin{tabular}{|c|c||r|r|r|r|r|r|r|r|l|}
    \hline
% Name Agg Traces             Hop   Router   Excl.   Router Excl.    Diam-
%                  Target   Router    BGP    Router   ASNs  Router   eter
%		    Addrs    Addrs  Pfxs.    BGP            ASNs   95thPerc
    {\textbf{Yarrp}} & \multirow{3}{*}{\textbf{Agg}} & \multirow{3}{*}{\textbf{Traces}} & {\textbf{Target}} &  {\textbf{Hop}} & {\textbf{Rtr}} &{\textbf{Excl.}} & {\textbf{Rtr}} & {\textbf{Excl.}} & {\textbf{Path Len}} & {\bf Reach} \\
     {\bf Campaign} &  & & {\textbf{Addrs}} & {\textbf{Rtr}} & {\textbf{BGP}} & {\bf Rtr} & {\bf ASNs} & {\bf Rtr} & {\bf {95} Perc.} & {\bf Target} \\
     vantage targs &  & & & {\bf Addrs} & {\bf Pfxs.} & {\bf BGP} & & {\bf ASNs} & {\bf (Median)} & {\bf ASN} \\
    \hline\hline
% { AUTOMATICALLY GENERATED - DO NOT EDIT DATA LINES BELOW:
EU-NET cdn k32 & z64 & 3.2M & 3.2M & 694.4k & 1.9k & 23  & 1.1k & 6  & {15} (9)  &  54\% \\ \hline
US-EDU-1 cdn k32 & z64 & 3.2M & 3.2M & 677.3k & 1.9k & 6  & 1.1k & 0  & {16} (11)  &  54\% \\ \hline
EU-NET tum & z64 & 2.1M & 2.1M & 502.2k & 7.6k & 127  & 5.8k & 66  & {16} (7)  &  70\% \\ \hline
US-EDU-1 tum & z64 & 2.1M & 2.1M & 491.8k & 7.5k & 29  & 5.7k & 10  & {18} (10)  &  68\% \\ \hline
US-EDU-2 tum & z64 & 2.1M & 2.1M & 424.1k & 5.8k & 78  & 4.4k & 55  & {20} (15)  &  51\% \\ \hline
US-EDU-2 cdn k32 & z64 & 3.2M & 3.2M & 390.4k & 1.3k & 2  & 780  & 1  & {19} (16)  &  47\% \\ \hline
EU-NET cdn k32 & z48 & 524.1k & 524.1k & 185.2k & 1.7k & 18  & 1.1k & 5  & {15} (9)  &  74\% \\ \hline
US-EDU-1 cdn k32 & z48 & 524.2k & 524.2k & 184.7k & 1.7k & 1  & 1.1k & 0  & {16} (11)  &  75\% \\ \hline
EU-NET fdns & z64 & 739.7k & 739.7k & 150.0k & 6.0k & 88  & 4.8k & 47  & {13} (5)  &  53\% \\ \hline
US-EDU-1 fdns & z64 & 746.9k & 746.9k & 147.5k & 5.9k & 18  & 4.8k & 6  & {16} (9)  &  53\% \\ \hline
EU-NET dnsdb & z64 & 232.7k & 232.7k & 124.1k & 7.5k & 129  & 5.8k & 72  & {17} (9)  &  63\% \\ \hline
US-EDU-1 dnsdb & z64 & 233.0k & 233.0k & 121.9k & 7.4k & 25  & 5.7k & 11  & {19} (12)  &  63\% \\ \hline
US-EDU-2 fdns & z64 & 746.9k & 746.9k & 117.1k & 4.1k & 41  & 3.4k & 27  & {21} (15)  &  39\% \\ \hline
EU-NET 6gen & z64 & 4.4M & 4.4M & 108.6k & 6.8k & 133  & 5.0k & 61  & {32} (8)  &  30\% \\ \hline
US-EDU-2 cdn k32 & z48 & 524.2k & 524.2k & 107.3k & 1.1k & 2  & 738  & 2  & {20} (16)  &  61\% \\ \hline
US-EDU-1 6gen & z64 & 4.5M & 4.5M & 105.8k & 6.7k & 35  & 5.0k & 13  & {32} (10)  &  29\% \\ \hline
EU-NET cdn k256 & z64 & 396.7k & 396.7k & 105.7k & 1.2k & 8  & 614  & 1  & {15} (9)  &  53\% \\ \hline
US-EDU-1 cdn k256 & z64 & 396.7k & 396.7k & 103.8k & 1.1k & 1  & 605  & 0  & {15} (10)  &  54\% \\ \hline
EU-NET tum & z48 & 346.1k & 346.1k & 99.8k & 6.3k & 97  & 4.8k & 50  & {16} (5)  &  44\% \\ \hline
US-EDU-1 tum & z48 & 362.7k & 362.7k & 99.0k & 6.2k & 18  & 4.8k & 5  & {16} (7)  &  42\% \\ \hline
US-EDU-2 dnsdb & z64 & 233.0k & 233.0k & 80.6k & 5.0k & 69  & 4.0k & 49  & {22} (16)  &  39\% \\ \hline
EU-NET cdn k256 & z48 & 162.4k & 162.4k & 80.2k & 1.1k & 11  & 608  & 1  & {15} (9)  &  73\% \\ \hline
US-EDU-1 cdn k256 & z48 & 162.4k & 162.4k & 79.8k & 1.0k & 0  & 599  & 0  & {16} (11)  &  75\% \\ \hline
US-EDU-2 6gen & z64 & 4.5M & 4.5M & 79.6k & 4.9k & 74  & 3.7k & 41  & {24} (15)  &  22\% \\ \hline
US-EDU-2 tum & z48 & 362.7k & 362.7k & 78.3k & 4.7k & 57  & 3.7k & 42  & {20} (15)  &  36\% \\ \hline
EU-NET fdns & z48 & 216.0k & 216.0k & 75.0k & 4.6k & 61  & 3.8k & 29  & {13} (5)  &  34\% \\ \hline
US-EDU-1 fdns & z48 & 228.7k & 228.7k & 74.0k & 4.6k & 12  & 3.8k & 4  & {14} (5)  &  31\% \\ \hline
EU-NET dnsdb & z48 & 93.6k & 93.6k & 71.7k & 6.1k & 95  & 4.8k & 50  & {17} (8)  &  57\% \\ \hline
US-EDU-1 dnsdb & z48 & 93.8k & 93.8k & 70.4k & 6.0k & 21  & 4.7k & 9  & {20} (11)  &  56\% \\ \hline
US-EDU-2 cdn k256 & z64 & 396.7k & 396.7k & 58.0k & 762  & 0  & 418  & 0  & {20} (16)  &  46\% \\ \hline
EU-NET 6gen & z48 & 1.4M & 1.4M & 57.7k & 6.3k & 93  & 4.7k & 52  & {32} (7)  &  18\% \\ \hline
US-EDU-2 fdns & z48 & 228.7k & 228.7k & 56.9k & 3.1k & 30  & 2.6k & 19  & {19} (15)  &  23\% \\ \hline
US-EDU-1 6gen & z48 & 1.4M & 1.4M & 56.6k & 6.2k & 22  & 4.7k & 10  & {32} (10)  &  18\% \\ \hline
EU-NET caida & z64 & 104.4k & 104.4k & 48.5k & 6.0k & 94  & 4.6k & 52  & {32} (8)  &  29\% \\ \hline
US-EDU-1 caida & z64 & 105.2k & 105.2k & 48.1k & 5.9k & 30  & 4.6k & 13  & {32} (10)  &  29\% \\ \hline
EU-NET caida $\ast$ & z64 & 104.4k & 104.4k & 47.7k & 5.9k & 105  & 4.5k & 57  & {32} (9)  &  37\% \\ \hline
US-EDU-1 caida $\ast$ & z64 & 105.2k & 105.2k & 47.1k & 5.8k & 19  & 4.5k & 9  & {31} (11)  &  36\% \\ \hline
EU-NET caida & z48 & 77.7k & 77.7k & 46.2k & 5.9k & 92  & 4.5k & 51  & {32} (8)  &  28\% \\ \hline
US-EDU-2 dnsdb & z48 & 93.8k & 93.8k & 46.2k & 4.1k & 56  & 3.3k & 40  & {22} (16)  &  34\% \\ \hline
US-EDU-1 caida & z48 & 78.3k & 78.3k & 45.6k & 5.8k & 19  & 4.5k & 7  & {31} (11)  &  28\% \\ \hline
US-EDU-2 cdn k256 & z48 & 162.4k & 162.4k & 44.5k & 680  & 0  & 405  & 0  & {20} (16)  &  59\% \\ \hline
EU-NET caida $\ast$ & z48 & 77.8k & 77.8k & 43.4k & 5.4k & 97  & 4.3k & 53  & {32} (9)  &  38\% \\ \hline
US-EDU-1 caida $\ast$ & z48 & 78.3k & 78.3k & 42.8k & 5.3k & 18  & 4.2k & 8  & {31} (11)  &  37\% \\ \hline
EU-NET fiebig & z64 & 773.4k & 773.4k & 41.3k & 3.2k & 34  & 2.8k & 23  & {11} (3)  &  35\% \\ \hline
US-EDU-1 fiebig & z64 & 1.0M & 1.0M & 39.6k & 3.1k & 11  & 2.7k & 6  & {14} (8)  &  26\% \\ \hline
US-EDU-2 6gen & z48 & 1.4M & 1.4M & 39.5k & 4.4k & 60  & 3.4k & 41  & {24} (15)  &  11\% \\ \hline
US-EDU-2 caida & z64 & 105.2k & 105.2k & 32.2k & 4.2k & 66  & 3.3k & 47  & {23} (15)  &  21\% \\ \hline
US-EDU-2 caida $\ast$ & z64 & 105.2k & 105.2k & 31.8k & 4.1k & 88  & 3.2k & 46  & {23} (15)  &  27\% \\ \hline
US-EDU-2 fiebig & z64 & 1.0M & 1.0M & 30.5k & 2.4k & 17  & 2.1k & 13  & {18} (13)  &  15\% \\ \hline
US-EDU-2 caida & z48 & 78.3k & 78.3k & 30.2k & 4.0k & 56  & 3.1k & 41  & {23} (15)  &  19\% \\ \hline
US-EDU-2 caida $\ast$ & z48 & 78.3k & 78.3k & 28.3k & 3.7k & 71  & 3.0k & 37  & {22} (15)  &  26\% \\ \hline
EU-NET fiebig & z48 & 66.0k & 66.0k & 16.9k & 2.5k & 25  & 2.2k & 16  & {12} (3)  &  19\% \\ \hline
US-EDU-1 fiebig & z48 & 102.2k & 102.2k & 16.6k & 2.5k & 6  & 2.2k & 2  & {16} (2)  &  12\% \\ \hline
US-EDU-2 fiebig & z48 & 102.2k & 102.2k & 10.8k & 1.7k & 14  & 1.5k & 10  & {19} (4)  &  6\% \\ \hline
% }
  \end{tabular}
  \end{center}
\end{table*}


==> results_validation_table_scaled.tex <==

% DO NOT EDIT MANUALLY!
% CREATED AUTOMATICALLY FROM "results_validation_table.tex"

\begin{table*}[t]
  \caption{Comparing Yarrp results to a CDN's proprietary prober results (one vantage, multiple servers).}
  \vspace{-4mm}
  \begin{center}
  \begin{tabular}{|c|c||r|r|r|r|r|r|r|r|l|}
    \hline
% Name Agg Traces             Hop   Router   Excl.   Router Excl.    Diam-
%                  Target   Router    BGP    Router   ASNs  Router   eter
%		    Addrs    Addrs  Pfxs.    BGP            ASNs   95thPerc
    {\bf Yarrp vs. {\em CDN}} & \multirow{3}{*}{\textbf{Agg}} & \multirow{3}{*}{\textbf{Traces}} & {\textbf{Target}} &  {\textbf{Hop}} & {\textbf{Rtr}} &{\textbf{Excl.}} & {\textbf{Rtr}} & {\textbf{Excl.}} & {\textbf{Path Len}} & {\bf Reach} \\
     {\bf Campaign} &  & & {\textbf{Addrs}} & {\textbf{Rtr}} & {\textbf{BGP}} & {\bf Rtr} & {\bf ASNs} & {\bf Rtr} & {\bf {95} Perc.} & {\bf Target} \\
     vantage targs &  & & & {\bf Addrs} & {\bf Pfxs.} & {\bf BGP} & & {\bf ASNs} & {\bf (Median)} & {\bf ASN} \\
    \hline\hline
% { AUTOMATICALLY GENERATED - DO NOT EDIT DATA LINES BELOW:
{\em CDN cdn k32} & z64 & 3.1M & 3.1M & 764.9k & 1.8k & 27  & 1.0k & 4  & {17} (10)  &  55\% \\ \hline
\hline
ALL cdn k32 & z64 & 9.6M & 3.2M & 756.6k & 2.0k & 31  & 1.2k & 7  & {18} (12)  &  52\% \\ \hline
\hline
EU-NET cdn k32 & z64 & 3.2M & 3.2M & 694.4k & 1.9k & 23  & 1.1k & 6  & {15} (9)  &  54\% \\ \hline
US-EDU-1 cdn k32 & z64 & 3.2M & 3.2M & 677.3k & 1.9k & 6  & 1.1k & 0  & {16} (11)  &  54\% \\ \hline
US-EDU-2 cdn k32 & z64 & 3.2M & 3.2M & 390.4k & 1.3k & 2  & 780  & 1  & {19} (16)  &  47\% \\ \hline
% }
  \end{tabular}
  \end{center}
\end{table*}

